Towards Practical Differential Privacy for SQL Queries

Differential privacy promises to enable general data analytics while protecting individual privacy, but existing differential privacy mechanisms do not support the wide variety of features and databases used in real-world SQL-based analytics systems. This paper presents the first practical approach for differential privacy of SQL queries. Using 8.1 million real-world queries, we conduct an empirical study to determine the requirements for practical differential privacy, and discuss limitations of previous approaches in light of these requirements. To meet these requirements we propose elastic sensitivity, a novel method for approximating the local sensitivity of queries with general equijoins. We prove that elastic sensitivity is an upper bound on local sensitivity and can therefore be used to enforce differential privacy using any local sensitivity-based mechanism. We build FLEX, a practical end-to-end system to enforce differential privacy for SQL queries using elastic sensitivity. We demonstrate that FLEX is compatible with any existing database, can enforce differential privacy for real-world SQL queries, and incurs negligible (0.03%) performance overhead.

==> figures/running_example.tex <==
\begin{figure}%[!htb]
\centering

%\minipage{0.58\textwidth}
\small
\begin{lstlisting}[language=sql,numbers=left,morekeywords={with}]
WITH t1 AS
  (SELECT * FROM trips t JOIN cities c
	      ON t.city_id = c.id
    WHERE country = "USA")
SELECT city_name, SUM(trip_distance) AS total_miles
FROM t1
GROUP BY 1
\end{lstlisting}
%\endminipage
%\minipage{0.38\textwidth}

\scriptsize

\noindent \begin{tabular}{l l}
\minipage{0.23\textwidth}
\texttt{\texttt{trips}}:

\begin{tabular}{l|l|l}
  \textbf{trip\_id} & \textbf{city\_id} & \textbf{trip\_distance}\\
  \hline
  12345    & 1    & 2.6 \\
  12346    & 1    & 1.3 \\
  12347    & 2    & 2.1 \\
\end{tabular}
\endminipage
&
%\vspace{2mm}

\minipage{0.23\textwidth}
\texttt{\texttt{cities}}:

\begin{tabular}{l|l|l}
  \textbf{id} & \textbf{city\_name} & \textbf{country} \\
  \hline
  1    & San Francisco  & USA \\
  2    & New York       & USA \\
  3    & London         & UK \\
\end{tabular}
\endminipage
\end{tabular}

%\endminipage
\caption{Running example query and data: Calculate cumulative miles
  driven per U.S. city.}\label{fig:running-example}
%\vspace*{4mm}
\end{figure}




==> figures/running_example_ast.tex <==
%\begin{figure}
\begin{lstlisting}[
    basicstyle=\tiny\fontfamily{zi4}\selectfont,
	%basicstyle=\small\ttfamily\color{xanadu},
	keywordstyle=\color{black},
	    tabsize=2,
	    numbers=left,
	xleftmargin=2mm
]
Query
	With
		Name["t1"]
	Query
		QuerySpecification
			Select
				QualifiedName["city_name"]
			From
				Join
					Alias["t"]
						Table["trips"]
					Alias["c"]
						Table["cities"]
				Condition
					EQUAL
						Dereference
							Table["t"]
							Name["city_id"]
						Dereference
							Table["c"]
							Name["city_id"]
			Where
				EQUAL
					QualifiedName["city_id"]
					String["USA"]
	QuerySpecification
		Select
			QualifiedName["city_name"]
			Alias["total_miles"]
				FunctionCall["sum"]
					QualifiedName["trip_distance"]
		From
			Table["t1"]
		GroupBy
			Long[1]
\end{lstlisting}
\caption{AST for the running example.}\label{fig:running-example-ast}
%\end{figure}

